Generalized Rogers Ramanujan Expressions for Some Non--Singlet Twisted Affine Algebras

Hatayama et al. described generalized Rogers--Ramanujan (GRR) expressions for the string functions of the singlet representation of twisted affine algebras. We give here such GRR expressions for some non-singlet string functions. In the case of the algebra $A_2^{(2)}$ this gives all the string functions. We verify these expressions using Freudenthal--Kac formula.

==> phyzzx.fonts.tex <==
%
% PHYZZX fonts are kept in this separate file
% in order to facilitate font substitution.
%
% This file should be called PHYZZX.FONTS on sites using CM fonts
% and PHYZZX.CMFONTS on other sites.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\font\teniu=cmu10
\font\seventeenrm =cmr12 scaled\magstep2
\font\fourteenrm  =cmr12 scaled\magstep1
\font\twelverm    =cmr10 scaled\magstep1
\font\tenrm       =cmr8  scaled\magstep1
\font\ninerm      =cmr7  scaled\magstep1
\font\sevenrm     =cmr6  scaled\magstep1
\font\sixrm       =cmr5  scaled\magstep1
\let\fiverm=\sixrm        % no cmr4
%
\font\seventeenbf =cmbx12 scaled\magstep2
\font\fourteenbf  =cmbx12 scaled\magstep1
\font\twelvebf    =cmbx10 scaled\magstep1
\font\tenbf       =cmbx8  scaled\magstep1
\font\ninebf      =cmbx7  scaled\magstep1
\font\sevenbf     =cmbx6  scaled\magstep1
\font\sixbf       =cmbx5  scaled\magstep1
\let\fivebf=\sixbf        % no cmbx4
%
\font\seventeeni  =cmmi12 scaled\magstep2    \skewchar\seventeeni='177
\font\fourteeni   =cmmi12 scaled\magstep1     \skewchar\fourteeni='177
\font\twelvei     =cmmi10 scaled\magstep1       \skewchar\twelvei='177
\font\teni        =cmmi8  scaled\magstep1          \skewchar\teni='177
\font\ninei       =cmmi7  scaled\magstep1         \skewchar\ninei='177
\font\seveni      =cmmi6  scaled\magstep1        \skewchar\seveni='177
\font\sixi        =cmmi5  scaled\magstep1          \skewchar\sixi='177
\let\fivei=\sixi          % no cmmi4
%
\font\seventeensy =cmsy10 scaled\magstep3    \skewchar\seventeensy='60
\font\fourteensy  =cmsy10 scaled\magstep2     \skewchar\fourteensy='60
\font\twelvesy    =cmsy10 scaled\magstep1       \skewchar\twelvesy='60
\font\tensy       =cmsy8  scaled\magstep1          \skewchar\tensy='60
\font\ninesy      =cmsy7  scaled\magstep1         \skewchar\ninesy='60
\font\sevensy     =cmsy6  scaled\magstep1        \skewchar\sevensy='60
\font\sixsy       =cmsy5  scaled\magstep1          \skewchar\sixsy='60
\let\fivesy=\sixsy        % no cmsy4
%
\font\seventeenex =cmex10 scaled\magstep3
\font\fourteenex  =cmex10 scaled\magstep2
\font\twelveex    =cmex10 scaled\magstep1
\let\tenex=\twelveex
%
\font\seventeensl =cmsl12 scaled\magstep2
\font\fourteensl  =cmsl12 scaled\magstep1
\font\twelvesl    =cmsl10 scaled\magstep1
\font\tensl       =cmsl8  scaled\magstep1
\let\ninesl=\ninerm     % no cmsl7
%
\font\seventeenit =cmti12 scaled\magstep2
\font\fourteenit  =cmti12 scaled\magstep1
\font\twelveit    =cmti10 scaled\magstep1
\font\tenit       =cmti8  scaled\magstep1
\font\nineit      =cmti7  scaled\magstep1
%
\font\fourteentt  =cmtt12 scaled\magstep1
\font\twelvett    =cmtt10 scaled\magstep1
\font\tentt       =cmtt8  scaled\magstep1
%
\font\fourteencp  =cmcsc10 scaled\magstep2
\font\twelvecp    =cmcsc10 scaled\magstep1
\let\tencp=\twelvecp      % no cmcsc8
%
\font\tenmsa=msam8 scaled\magstep1
\font\sevenmsa=msam6 scaled\magstep1
\font\fivemsa=msam5 scaled\magstep1
\font\tenmsb=msbm8 scaled\magstep1
\font\sevenmsb=msbm6 scaled\magstep1
\font\fivemsb=msbm5 scaled\magstep1
\font\teneufm=eufm8 scaled\magstep1
\font\seveneufm=eufm6 scaled\magstep1
\font\fiveeufm=eufm5 scaled\magstep1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\fourteenf@nts{\relax
    \textfont0=\fourteenrm          \scriptfont0=\tenrm
      \scriptscriptfont0=\sevenrm
    \textfont1=\fourteeni           \scriptfont1=\teni
      \scriptscriptfont1=\seveni
    \textfont2=\fourteensy          \scriptfont2=\tensy
      \scriptscriptfont2=\sevensy
    \textfont3=\fourteenex          \scriptfont3=\twelveex
      \scriptscriptfont3=\tenex
    \textfont\itfam=\fourteenit     \scriptfont\itfam=\tenit
    \textfont\slfam=\fourteensl     \scriptfont\slfam=\tensl
    \textfont\bffam=\fourteenbf     \scriptfont\bffam=\tenbf
      \scriptscriptfont\bffam=\sevenbf
    \textfont\ttfam=\fourteentt
    \textfont\cpfam=\fourteencp }
%
\def\twelvef@nts{\relax
    \textfont0=\twelverm          \scriptfont0=\ninerm
      \scriptscriptfont0=\sixrm
    \textfont1=\twelvei           \scriptfont1=\ninei
      \scriptscriptfont1=\sixi
    \textfont2=\twelvesy          \scriptfont2=\ninesy
      \scriptscriptfont2=\sixsy
    \textfont3=\twelveex          \scriptfont3=\tenex
      \scriptscriptfont3=\tenex
    \textfont\itfam=\twelveit     \scriptfont\itfam=\nineit
    \textfont\slfam=\twelvesl     \scriptfont\slfam=\ninesl
    \textfont\bffam=\twelvebf     \scriptfont\bffam=\ninebf
      \scriptscriptfont\bffam=\sixbf
    \textfont\ttfam=\twelvett
    \textfont\cpfam=\twelvecp }
%
\def\tenf@nts{\relax
    \textfont0=\tenrm          \scriptfont0=\sevenrm
      \scriptscriptfont0=\fiverm
    \textfont1=\teni           \scriptfont1=\seveni
      \scriptscriptfont1=\fivei
    \textfont2=\tensy          \scriptfont2=\sevensy
      \scriptscriptfont2=\fivesy
    \textfont3=\tenex          \scriptfont3=\tenex
      \scriptscriptfont3=\tenex
    \textfont\itfam=\tenit     \scriptfont\itfam=\seveni  % no \sevenit
    \textfont\slfam=\tensl     \scriptfont\slfam=\sevenrm % no \sevensl
    \textfont\bffam=\tenbf     \scriptfont\bffam=\sevenbf
      \scriptscriptfont\bffam=\fivebf
    \textfont\ttfam=\tentt
    \textfont\cpfam=\tencp }


==> phyzzx.local.tex <==
%
%  This is the PHYZZX.LOCAL file.
%  It contains local, ie. site-dependent macros.
%
%  This version of the file is for use at SLAC only.
%  Do not use it as is at other sites -- it is distributed only
%  to provide an example of macros you may want to use at your site.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\slacpub{\afterassignment\slacp@b\toks@}
\def\slacp@b{\edef\n@xt{\Pubnum={SLAC--PUB--\the\toks@}}\n@xt}
\let\pubnum=\slacpub
%
\expandafter\ifx\csname eightrm\endcsname\relax
    \let\eightrm=\ninerm \let\eightbf=\ninebf \fi
%
\def\memohead{\hrule height\z@ \kern -0.5in
    \line{\quad\fourteenrm SLAC MEMORANDUM\hfil \twelverm\the\date\quad}}
\def\memorule{\par \medskip \hrule height 0.5pt \kern 1.5pt
   \hrule height 0.5pt \medskip}
%
\def\SLACHEAD{\setbox0=\vtop{\baselineskip=10pt
     \ialign{\eightrm ##\hfil\cr
        \slacbin\cr
        P.^O.^Box 4349\cr
        Stanford, CA 94309\cropen{1\jot}
        \slacphone\cr }}%
   \setbox2=\hbox{\caps Stanford Linear Accelerator Center}%
   \hrule height \z@ \kern -0.5in
   \vbox to 0pt{\vss\centerline{\seventeenrm STANFORD UNIVERSITY}}
   \vbox{} \medskip
   \line{\hbox to 0.7\hsize{\hss \lower 10pt \box2 \hfill }\hfil
         \hbox to 0.25\hsize{\box0 \hfil }}\medskip }
\let\letterhead=\SLACHEAD
%
\FromAddress={\crcr \slacbin \cr
    P.\ O.\ Box 4349\cr Stanford, California 94309\cr }
%
\def\slacbin{SLAC\expandafter\ifx\csname binno\endcsname\relax
                             \else , Bin \binno \fi }
\def\slacphone{(415) 926--\slacext}
\def\slacext{3300}
%
\def\doeack{\foot{Work supported by the Department of Energy,
      contract DE--AC03--76SF00515.}}
%
\VOFFSET=33pt
\papersize
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Now comes the graphic package.
%  This version is rather primitive
%
\newwrite\figscalewrite
\newif\iffigscaleopen
\newif\ifgrayscale
\newif\ifreadyfile
\def\picturedefault{\grayscalefalse \readyfilefalse
    \gdef\ready{\readyfiletrue}\gdef\gray{\ready\grayscaletrue}}
%
\def\parsefilename{\ifreadyfile \else
    \iffigscaleopen \else \gl@bal\figscaleopentrue
       \immediate\openout\figscalewrite=\jobname.scalecon \fi
    \toks0={ }\immediate\write\figscalewrite{%
       \the\p@cwd \the\toks0 \the\p@cht \the\toks0 \the\picfilename }%
    \expandafter\p@rse \the\picfilename..\endp@rse \fi }
%
\def\p@rse#1.#2.#3\endp@rse{%
   \if*#3*\dop@rse #1.1..\else \if.#3\dop@rse #1.1..\else
                                \dop@rse #1.#3\fi \fi
   \expandafter\picfilename\expandafter{\n@xt}}
\def\dop@rse#1.#2..{\count255=#2 \ifnum\count255<1 \count255=1 \fi
   \ifnum\count255<10  \edef\n@xt{#1.PICT00\the\count255}\else
   \ifnum\count255<100 \edef\n@xt{#1.PICT0\the\count255}\else
                       \edef\n@xt{#1.PICT\the\count255}\fi\fi }
%
\def\redopicturebox{\edef\picturedefinition{\ifgrayscale
     \special{insert(\the\picfilename)}\else
     \special{mergeug(\the\picfilename)}\fi }}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Few miscellaneous macros
%
\let\us=\undertext
\let\rule=\memorule
\let\eqnalign=\eqname
%
\def\pri{^{\, \prime }}
\def\prii{^{\, \prime\, \prime }}
\def\priii{^{\, \prime\, \prime\, \prime }}
\def\epem{{e^+e^-}}
%%
\def\larrow{\leftarrow}
\def\rarrow{\rightarrow }
\def\uarrow{\uparrow }
\def\darrow{\downarrow }
\def\dblarrow{\doublearrow }
\def\longvec{\overrightarrow }
\def\wtilde{\widetilde }
%%
\def\xplus{\becomes{x\rarrow{+\infty}}}
\def\xminus{\becomes{x\rarrow{-\infty}}}
\def\xxx{\becomes{x\rarrow\infty}}
%%
\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern3pt
\vbox{\kern3pt#1\kern3pt}\kern3pt\vrule}\hrule}}
%%

